Approximate Gaussian Elimination for Laplacians: Fast, Sparse, and Simple

We show how to perform sparse approximate Gaussian elimination for Laplacian matrices. We present a simple, nearly linear time algorithm that approximates a Laplacian by a matrix with a sparse Cholesky factorization, the version of Gaussian elimination for symmetric matrices. This is the first nearly linear time solver for Laplacian systems that is based purely on random sampling, and does not use any graph theoretic constructions such as low-stretch trees, sparsifiers, or expanders. The crux of our analysis is a novel concentration bound for matrix martingales where the differences are sums of conditionally independent variables.

==> basic-cholesky.tex <==
\subsection{Basic Cholesky Factorization}

{\color{blue}
Here we could have a section 
outlining the standard Cholesky factorization algorithm.
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:


==> definitions.tex <==
\subsection{Definitions}

For notational convenience, we define
\[
\truncX^{(i)} = \ind{\goodUntil_{i}} X^{(i)}
\]

We consider the sum $\truncX = \sum_{i = 1}^{k}
\truncX^{(i)} $.

\Rnote{For the following, maybe need to talk about filtrations, or how
  $\goodUntil$ is fixed based on the events we condition on}

\begin{definition}
  \textbf{ A {\seqsum}} is a sum of random Hermitian
  $d \times d$ matrices ${Z = \sum_{i = 1}^{k} Z^{(i)}}$,
   with the following structure:
 \begin{enumerate}
 \item \Rnote{TODO} Not clear if this is a little too complicated? Can we
     get rid of the $R_{i}$?
 \item \Rnote{TODO} Also not clear if the formal setup is quite right?
 \item There  there exists a sequence of random variables
  $(r_{1}, R_{1}), \ldots, (r_{k},R_{k})$, s.t. for all $j$,
  $Z^{(j)}$ is a deterministic function of
  $(r_{1}, R_{1}), \ldots, (r_{j},R_{j})$.
\item For all $j$, conditional on $(r_{1}, R_{1}), \ldots,
  (r_{j-1},R_{j-1})$ and $r_{j}$,
  $Z^{(j)}$ is a sum of independent random Hermitian matrices,
  $Z^{(j)}_{1}, \ldots,Z^{(j)}_{l}$, i.e.
 \[
  Z^{(j)} = \sum_{e = 1}^{l} Z^{(j)}_{e}
  \]
 \end{enumerate}
\end{definition}
We can think of $R_{j}$ as the source of randomness for the sum
$\sum_{e= 1}^{l} Z^{(j)}_{e}.$


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:

==> intro-ras.tex <==
\paragraph{Technical Contributions.}

To analyze our algorithm, we develop new concentration bounds for a class of matrix martingales.
We call these {\seqsum}s.
The name is motivated by a simple scalar model: at each step, we pick a random bag
of dice from a collection of bags (in the algorithm, this corresponds
to picking a random vertex to eliminate), and then we independently
roll each die in the selected bag (corresponding to drawing
independent samples from the clique added during elimination).
The concentration bound gives us a powerful tool for handling
conditionally independent sums of variables.

\Rnote{Should we address Mackey? Probably not? In that case, delete
  the next paragraph}

Our matrix concentration result has applications similar
to some of the cases addressed
by Mackey et al.~\cite{mackey2014matrix}, but while their theory has a
broad range of applications, 
we are able to handle
conditional indepence structures in the context of
martingales specifically,
without requiring the self-reproducing property used in their result.

\Rnote{I really don't know if that's right.
For one, they don't seem to handle general martingales at all?}

The sequential sampling used by our algorithm is not readily analyzable using
standard matrix concentration bounds, because the matrix we sample at each
step depends on heavily on random choices made in previous steps.
To solve this problem, we develop a technique called \emph{martingale
  truncation}, which essentially allows us to assume during analysis that the
martingale been well-behaved until the current step, which in turn
lets us establish the necessary control on the variance of the martingale to
prove concentration.

A third difficulty in analyzing our algorithm relates specifically to
the matrices generated by Cholesky factorization.
The factorization produces matrices that locally do not resemble the
input Laplacian matrix, making it difficult to bound the variance of the
sampling procedure.
We address this problem by choosing a random vertex to eliminate:
Using a global relation between the original Laplacian and the
partially factorized matrices, we can bound the variance of the sampling
procedure after randomizing the vertex we eliminate.

A key element of all previous Laplacian solvers is sophisticated
procedures for computing good sampling
probabilities.
In comparison, we are able to use very crude initial estimates.
We then maintain sufficiently good sampling probabilities
throughout the algorithm
by using local relationships between the edges removed by elimination
and the new edges introduced at the same time.
For Laplacians, a very strong local relation exists due to the
well-known fact that \emph{effective resistance} in Laplacians is a distance.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:


==> macros-other.tex <==


\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}

\newcommand\ttau{\boldsymbol{\tau}}
\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}
\newcommand\ddelta{\boldsymbol{\delta}}
\newcommand\eepsilon{\boldsymbol{\epsilon}}

\newcommand\er{R_{eff}}


\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
\newcommand\bbbar{\overline{\boldsymbol{\mathit{x}}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
\renewcommand\ll{\boldsymbol{\mathit{l}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\xxbar{\overline{\boldsymbol{\mathit{x}}}}
\newcommand\yybar{\overline{\boldsymbol{\mathit{y}}}}
\newcommand\zzbar{\overline{\boldsymbol{\mathit{z}}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\BBtil{\boldsymbol{\tilde{\mathit{B}}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\CChat{\boldsymbol{\widehat{\mathit{C}}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\EE{\boldsymbol{\mathit{E}}}
\newcommand\FF{\boldsymbol{\mathit{F}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\boldsymbol{\mathit{M}}}
\newcommand\MMbar{\overline{\boldsymbol{\mathit{M}}}}
\newcommand\Mtil{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\Ltil{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\TT{\boldsymbol{\mathit{T}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}



\newcommand\AAn{\boldsymbol{\mathcal{A}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}

\newcommand\AAhat{\boldsymbol{\widehat{\mathit{A}}}}
\newcommand\AAapprox{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDhat{\boldsymbol{\widehat{\mathit{D}}}}
\newcommand\DDapprox{\boldsymbol{\widetilde{\mathit{D}}}}
\newcommand\LLhat{\boldsymbol{\widehat{\mathit{L}}}}
\newcommand\LLapprox{\boldsymbol{\widetilde{\mathit{L}}}}
\newcommand\MMhat{\boldsymbol{\widehat{\mathit{M}}}}
\newcommand\MMtil{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\MMapprox{\boldsymbol{\widetilde{\mathit{M}}}}
\newcommand\UUhat{\boldsymbol{\widehat{\mathit{U}}}}

\newcommand\xxhat{\boldsymbol{\widehat{\mathit{x}}}}
\newcommand\bbhat{\boldsymbol{\widehat{\mathit{b}}}}


\newcommand\AAtil{\boldsymbol{\widetilde{\mathit{A}}}}
\newcommand\DDtil{\boldsymbol{\widetilde{\mathit{D}}}}

\newcommand\xxtil{\boldsymbol{\tilde{\mathit{x}}}}


\newcommand\Otil{\widetilde{O}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\Ghat{{\widehat{{G}}}}
\newcommand\Vhat{{\widehat{{V}}}}
\newcommand\Ehat{{\widehat{{E}}}}
\newcommand\ddhat{{\hat{\dd}}}
\newcommand\dhat{{\hat{{d}}}}
\newcommand\nhat{{\hat{{n}}}}
\def\Gtil{\widetilde{G}}

\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\newcommand{\nfrac}{\nicefrac}

==> multi-edge-dedup.tex <==
\section{Data Structures for Multi-Edges}
\label{sec:data-structure}

The pseudo-code in Algorithm\Rnote{TODO} does not address how to
implement the linear algebra in time linear in the number of non-zero
entries.
We briefly sketch how this can be achieved:
\Rnote{This language is awful!}
For each vertex $v$, we store a column vector of multi-edges
corresponding to the Laplacians $L_{\setof{u,v}}$ that we have found.
Each multi-edge is given by
\begin{itemize}
\item A destination $u$.
\item A weight $w$.
\item The leverage score upper bound $t$ \Rnote{need to
    deal with this being multi-edge too!}.
\end{itemize}
We do not store the multi-edge in both the column for $u$ and the
column for $v$. Instead, if $\pi(v) < \pi(u)$, we store the multi-edge
at $v$ (and vice versa).
This multi-edge structure makes it easy to append samples produced by
$\csamp$.
We just append each multi-edge sample output by $\csamp$ to the
appropriate column of multi-edges.
One issue remains:
The $\csamp$ procedure cannot accept multi-edge input, so we have to
produce a version of the column vector for $v$, where there is only
one entry for each destination $u$.
To do so, we allocate at the beginning of the $\cholesky$ algorithm
two arrays $\textsc{WeightDedup}$ and $\textsc{LeverageDedup}$, each of size $n$.
Each entry should initially be set to zero.
To de-duplicate the column vector of multi-edges for $v$,
we first pass once through the column vector,
and for each destination $u$, we increment $\textsc{WeightDedup}[u]$
by $w$, and increment $\textsc{LeverageDedup}[u]$ by $t$.
We then pass through the column vector for $v$ again, and create a
new column vector for $v$: When we process a multi-edge with
destination $u$, we append
$(u,\textsc{WeightDedup}[u],\textsc{LeverageDedup}[u])$ to the new
column vector unless $\textsc{WeightDedup}[u] == 0$, and then we set
$\textsc{WeightDedup}[u] \assign 0$ and $\textsc{LeverageDedup}[u]
\assign 0$, so that later multi-edges with destination $u$ will not be
appended to the new column vector for $v$.
We then pass this new column vector for $v$ to $\csamp$.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:


==> richardson.tex <==
\subsection{Richardson}

{\color{blue}
Here we should write a very short lemma on Richardson?
\\
Although, maybe it needs to appear in introduction?
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:


==> running-time.tex <==
\subsection{Running Time - or at least edge sample count}

Heuristically?
We're using $\beta = O(\log^{2}(n))$.
We should be maintaining that density?
\begin{enumerate}
\item $O(m \log n + n \log^{3} n)$ ish?
\item Or maybe $O(m \log^{3})$?
\item Or maybe $O(m \log n + n \log^{2} n)$
\item Or maybe $O(m + n \log^{2} n)$ in the best case?
\end{enumerate}

Oh, I think sparsifying along the way gives $O(m + \beta^{-1} n) = O(m + n
\log^{2} n)$. Although, there's stuff with the $\omega$ to be worked
out there.

And, we choose variable $\beta$, it might go down to $O(m + n \log^{1}
n)$?

\vspace{1 em}
%
\emph{OK, a sketch on the board gives edge count touched: $O(m \log n + n \log^{3} n)$.}
How? Assume $\eps$ is a fixed constant.
First, let's see a \emph{non-rigorous} argument:
Because, ignoring decay in edge count,
the edges added by sampling sum to $O(i \beta^{-1})$ in step $i$ (using the
fixed-$\beta$ algorithm).
So the expected degree of the eliminated vertex at step $i$ is 
$O( (m + i\log^{2}n) / (n-i) ) \leq O( (m + i\log^{2}n) / (n-i) )$. 
Summed over all $i$, we get $O(m\log n + n \log^{3}n)$.
Note: the fact that we only select vertices with low impact could
double the expected degree, but that's hidden by the big-O.

\vspace{1 em}

But: if we actually know the Reff, we'd just want to sparsify first.
And: if we use the increasing-$\epsilon$ trick, and sparsify between
each phase, where a phase halves the vertex count, then we should get
$\log^2 n$ edges from the sampling rate, and elim $n/2$ vertices.
And, with $n\log n$ original edges.
And then we hope for geometric decay from then onwards.
So ideally, we get edge count of $O(n\log^2n)$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "schur-lapsolver"
%%% End:

==> seqsum-definitions.tex <==
\subsection{Definitions}

For notational convenience, we define
\[
\truncX^{(i)} = \ind{\goodUntil_{i}} X^{(i)}
\]

We consider the sum $\truncX = \sum_{i = 1}^{k}
\truncX^{(i)} $.

\Rnote{For the following, maybe need to talk about filtrations, or how
  $\goodUntil$ is fixed based on the events we condition on}

\begin{definition}
  \textbf{ A {\seqsum}} is a sum of random Hermitian
  $d \times d$ matrices ${Z = \sum_{i = 1}^{k} Z^{(i)}}$,
   with the following structure:
 \begin{enumerate}
 \item \Rnote{TODO} Not clear if this is a little too complicated? Can we
     get rid of the $R_{i}$?
 \item \Rnote{TODO} Also not clear if the formal setup is quite right?
 \item There  there exists a sequence of random variables
  $(r_{1}, R_{1}), \ldots, (r_{k},R_{k})$, s.t. for all $j$,
  $Z^{(j)}$ is a deterministic function of
  $(r_{1}, R_{1}), \ldots, (r_{j},R_{j})$.
\item For all $j$, conditional on $(r_{1}, R_{1}), \ldots,
  (r_{j-1},R_{j-1})$ and $r_{j}$,
  $Z^{(j)}$ is a sum of independent random Hermitian matrices,
  $Z^{(j)}_{1}, \ldots,Z^{(j)}_{l_j}$, i.e.
 \[
  Z^{(j)} = \sum_{e = 1}^{l_j} Z^{(j)}_{e}
  \]
 \end{enumerate}
\end{definition}
We can think of $R_{j}$ as the source of randomness for the sum
$\sum_{e= 1}^{l_j} Z^{(j)}_{e}.$


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "simple-solver"
%%% End:
